An $H\alpha$ Imaging Survey of the all (Ultra-)Luminous Infrared Galaxies at $Dec. \ge -30^{\circ}$ in the GOALS Sample

This paper presents the result of $H\alpha$ imaging for luminous infrared galaxies (LIRGs) and ultra-luminous infrared galaxies (ULIRGs). \textbf{It is } a \textbf{complete subsample of Great Observatories All-sky LIRG Survery (GOALS) with $Dec. \ge -30^{\circ}$}, \textbf{and} consists 148 galaxies with $log(L_{IR}/L_{\odot}) \ge 11.0$. All the $H\alpha$ images were carried out using the 2.16-m telescope \textbf{at the Xinglong Station of the} National Astronomy Observatories, Chinese Academy of Sciences\textbf{ (NAOC),} during the year from 2006 to 2009. We obtained pure $H\alpha$ luminosity for each galaxy and corrected the luminosity for $[NII]$ emission, filter transmission and extinction. We also classified these galaxies based on their morphology and interaction. We found that the distribution of star-forming \textbf{regions} in these galaxies is related to this classification. As the merging process advanced, these galaxies tend to have a more compact distribution of star-forming region, higher \textbf{$L_{IR}$} and warmer IR-color ($f_{60}/f_{100}$). \textbf{These} results imply that the degree of dynamical disturbance plays an important role in determining the distribution of star-forming region.

==> AO_text.tex <==
\subsection{High-resolution Imaging}\label{subsec:hri}

As part of our standard process for validating transiting exoplanets, we observed EPIC~210693462 with infrared high-resolution adaptive optics (AO) imaging at Keck Observatory.  The Keck Observatory observations were made with the NIRC2 instrument on Keck-II behind the natural guide star AO system.  The observations were made on 2017~Aug~20 in the narrow-band $Br-\gamma$, the H-continuum, and J-continuum filters in the standard 3-point dither pattern that is used with NIRC2 to avoid the left lower quadrant of the detector which is typically noisier than the other three quadrants. The dither pattern step size was $3\arcsec$ and was repeated three times, with each dither offset from the previous dither by $0.5\arcsec$.  The observations utilized an integration time of 6.6, 4.0, and 2.903 seconds, respectively, with one coadd per frame for a total of 59.4, 36, and 3.92 seconds.  The camera was in the narrow-angle mode with a full field of view of $10\arcsec$ and a pixel scale of approximately $0.009942 \arcsec$ per pixel. The Keck AO observations clearly detected a nearly equal brightness companion approximately $0.8\arcsec$ to the southeast of the primary target. 

The NIRC2 AO data have a resolution of 0.049$^{\prime\prime}$ (FWHM) in the $Br$-$\gamma$ filter, 0.040$^{\prime\prime}$ (FWHM) in the $H$-$cont$, and 0.039$^{\prime\prime}$ (FWHM) in the $J$-$cont$ filter. The sensitivities of the AO data were determined by injecting fake sources into the final combined images with separations from the primary targets in integer multiples of the central source's FWHM \citep{furlan2017}.  The sensitivity curves shown in Figure \ref{fig:ao_contrast} represent the 5$\sigma$ limits of the imaging data. The companion separation was measured from the $Br$-$\gamma$ image and found to be $\Delta\alpha = 0.259\arcsec \pm 0.001\arcsec$ and $\Delta\delta = -0.746\arcsec \pm 0.001\arcsec$.  The presence of the blended companion must be taken into account to obtain the correct transit depth and planetary radius \citep{ciardi2015}.

The stars have blended 2MASS magnitudes of $J = 10.545 \pm 0.026$ mag, $H=9.946 \pm 0.020$ mag and $K_s = 9.724 \pm 0.023$ mag.  The stars have measured magnitude differences of $\Delta J = 4.97 \pm 0.04$ mag, $\Delta H = 4.96 \pm 0.03$ mag, and $\Delta K_s = 0.988 \pm 0.003$ mag. $Br$-$\gamma$ has a central wavelength that is sufficiently close to $Ks$ to enable the deblending of the 2MASS magnitudes into the two components.  The primary star has deblended real apparent magnitudes of $J_1 = 10.910 \pm 0.027$ mag, $H_1 = 10.313 \pm 0.021$ mag, and $Ks_1 = 10.0918 \pm 0.023$ mag, corresponding to $(J-H)_1 = 0.597 \pm 0.033$ mag and $(H-K_s)_1 = 0.221 \pm 0.031$ mag. The companion star has deblended real apparent magnitudes of $J_2 = 11.907 \pm 0.0269$ mag, $H = 11.303 \pm 0.021$ mag, and $Ks_2 = 11.079 \pm 0.023$ mag, corresponding to $(J-H)_2 = 0.604 \pm 0.033$ mag and $(H-K_s)_2 = 0.224 \pm 0.031$ mag. Utilizing the $(Kepmag - Ks)\ vs.\ (J-Ks)$ color relationships \citep{howell2012}, we derive approximate deblended Kepler magnitudes of the two components of $Kepmag_1 = 13.46\pm0.09$ mag and $Kepmag_1 = 14.49\pm0.10$ mag, for Kepler magnitude difference of $\Delta Kepmag = 1.03\pm0.12$ mag, which is used when fitting the light curves and deriving a true transit depth.

Both stars have infrared colors that are consistent with an M3V spectral type (Figure~\ref{fig:cc}).  It is unlikely that the star is a heavily reddened background star. Based upon an $R=3.1$ extinction law, an early-K star would have to be attenuated by more than 1 magnitude of extinction to make the star appear as a mid M-dwarf.  The entire line-of-sight extinction through the Galaxy is only $A_V\approx0.7$~mag at this location in the galaxy \citep{sf2011} making a background star an unlikely source of the detected companion. 

References used:

\bibitem[Ciardi et al.(2015)]{ciardi2015} Ciardi, D.~R., Beichman, C.~A., Horch, E.~P., \& Howell, S.~B.\ 2015, \apj, 805, 16 

\bibitem[Furlan et al.(2017)]{furlan2017} Furlan, E., Ciardi, D.~R., Everett, M.~E., et al.\ 2017, \aj, 153, 71

\bibitem[Howell et al.(2012)]{howell2012} Howell, S.~B., Rowe, J.~F., Bryson, S.~T., et al.\ 2012, \apj, 746, 123 

\bibitem[Schlafly \& Finkbeiner(2011)]{sf2011} Schlafly, E.~F., \& Finkbeiner, D.~P.\ 2011, \apj, 737, 103 




